Hypercurveball algorithm for sampling hypergraphs with fixed degrees

Comparative analysis between a network and a random graph model can uncover network properties that significantly deviate from those in random networks. The standard random graph model used for comparison uniformly samples random graphs with the same degrees as the network data, often achieved through edge-swap algorithms. However, for hypergraphs, fewer such methodologies are available. This study introduces the Hypercurveball algorithm, designed to sample random, potentially directed, hypergraphs with fixed degrees. Minor adjustments enable the sampling of hypergraphs without degenerate hyperedges, self-loops, or multi-hyperedges. For most of these algorithms, we prove whether they sample uniformly or with bias. We experimentally show that the Hypercurveball algorithm can be significantly faster or slower than the standard hyperedge-shuffling algorithm, which is the hyperedge-equivalent of the edge-swap algorithm. We present criteria on the hypergraph degree sequence that indicate when the Hypercurveball algorithm is more efficient than the standard hyperedge-shuffling method. Finally, our experimental results suggest polynomial scaling of the mixing time for both the Hypercurveball and hyperedge-shuffling algorithms.

==> proofs/uniformity.tex <==
To prove Theorem \ref{thm:uniform_sampling}, we first show that a hypertrade can always achieve a simple hyperedge shuffle in which only two elements in two different hyperedges exchange place. We then use the fact that the hyperedge-shuffle method leads to a strongly connected Markov Chain \cite{kraakman2024}, and that its proof only uses these simple hyperedge shuffles. 
\\
\begin{definition}[Simple hyperedge shuffle]
\label{def:simple}
    Let $e_1,e_2 \in E$ be two hyperedges. A hyperedge shuffle with $e_1$ and $e_2$ is simple if it modifies only two incidences, i.e., if it results in $e'_1$ and $e'_2$, where
    \begin{align*}
        e'_1 &= e_1 \backslash \{a\} \uplus \{b\}\\
        e'_2 &= e_2 \backslash \{b\} \uplus \{a\},        
    \end{align*}
    for some $a,b\in V$. For directed hypergraphs,
    \begin{align*}
        e^{\tail \prime}_1 &= e^{\tail}_1 \backslash \{a\} \uplus \{b\}\\
        e^{\tail \prime}_2 &= e^{\tail}_2 \backslash \{b\} \uplus \{a\}\\ 
        e^{\head \prime}_1 &= e^{\head}_1\\
        e^{\head \prime}_2 &= e^{\head}_2,
    \end{align*}
    or with tail and head swapped.
\end{definition}

A simple hyperedge shuffle only alters the incidences of two nodes. Therefore, it can be achieved using a hypertrade with those two nodes.
\\
\begin{lemma}
\label{lemma:simple}
Let a simple hyperedge shuffle on a hypergraph $H$ result in a hypergraph $H'$. There exists a hypertrade on $H$ that also results in $H'$.
\end{lemma}
\begin{proof}
    Let the simple hyperedge shuffle be as in Definition \ref{def:simple}. A hypertrade with $a$ and $b$ can result in $H'$ with
    \begin{align*}
        I_a(H') &= I_a(H) \backslash \{e_1\} \uplus \{e_2\}\\
        I_b(H') &= I_b(H) \backslash \{e_2\} \uplus \{e_1\},
    \end{align*}
    or with directed hypergraphs,
    \begin{align*}
        I^{\tail}_a(H') &= I^{\tail}_a(H) \backslash \{e_1\} \uplus \{e_2\}\\
        I^{\tail}_b(H') &= I^{\tail}_b(H) \backslash \{e_2\} \uplus \{e_1\}\\ 
        I^{\head}_a(H') &= I^{\head}_a(H)\\
        I^{\head}_b(H') &= I^{\head}_b(H).
    \end{align*}
\end{proof}

Using Lemma \ref{lemma:simple}, we prove Theorem \ref{thm:uniform_sampling}.

\begin{proof}[Proof of Theorem \ref{thm:uniform_sampling}]
    We prove the result for the directed hypergraph spaces $\mathcal{H}_{s,d,m}(\vb*{d}_2)$ and $\mathcal{H}_{s,m}(\vb*{d}_2)$. From these, the results for the undirected hypergraph spaces $\mathcal{H}_{d,m}(\vb*{d}_1)$ and $\mathcal{H}_{m}(\vb*{d}_1)$ follow directly. By Lemmas \ref{lemma:regular} and \ref{lemma:aperiodic}, the Markov chains underlying the Hypercurveball algorithms for $\mathcal{H}_{s,d,m}(\vb*{d}_2)$ and $\mathcal{H}_{s,m}(\vb*{d}_2)$ are regular and aperiodic. It remains to prove that they are strongly connected.

    For $\mathcal{H}_{s,d,m}(\vb*{d}_2)$, the result follows from Lemma 6.3 in \cite{kraakman2024}, which states that $\mathcal{G}(\mathcal{H}_{s,d,m}(\vb*{d}_2))$ is strongly connected when using hyperedge shuffles. The proof shows that hypergraphs in $\mathcal{H}_{s,d,m}(\vb*{d}_2)$ are connected via a path of simple hyperedge shuffles. By Lemma \ref{lemma:simple} in this work, they are connected via a path of hypertrades as well. 

    For $\mathcal{H}_{s,m}(\vb*{d}_2)$, the result follows from Lemma 6.4 in \cite{kraakman2024}, which states that $\mathcal{G}(\mathcal{H}_{s,m}(\vb*{d}_2))$ is strongly connected when using hyperedge shuffles. The proof shows that hypergraphs in $\mathcal{H}_{s,m}(\vb*{d}_2)$ are connected via a path of simple hyperedge shuffles. By Lemma \ref{lemma:simple} in this work, they are connected via a path of hypertrades as well. 
\end{proof}
